A Generative Model of People in Clothing

We present the first image-based generative model of people in clothing for the full body. We sidestep the commonly used complex graphics rendering pipeline and the need for high-quality 3D scans of dressed people. Instead, we learn generative models from a large image database. The main challenge is to cope with the high variance in human pose, shape and appearance. For this reason, pure image-based approaches have not been considered so far. We show that this challenge can be overcome by splitting the generating process in two parts. First, we learn to generate a semantic segmentation of the body and clothing. Second, we learn a conditional model on the resulting segments that creates realistic images. The full model is differentiable and can be conditioned on pose, shape or color. The result are samples of people in different clothing items and styles. The proposed model can generate entirely new people with realistic clothing. In several experiments we present encouraging results that suggest an entirely data-driven approach to people generation is possible.

==> figures/tikz_cnn.tex <==
% CNN design tools.
\usetikzlibrary{3d}
\newif\ifcuboidshade
\newif\ifcuboidemphedge
%\newif\ifcuboiddrawxmarks
%\newif\ifcuboiddrawymarks
\newif\ifcuboidlabels
\newif\ifcuboidfrontpic
\newif\ifcuboiddrawfront
\newif\ifcuboiddrawtop
\newif\ifcuboiddrawright

\tikzset{
  cuboid/.is family,
  cuboid,
  shiftx/.initial=0,
  shifty/.initial=0,
  dimx/.initial=3,
  dimy/.initial=3,
  dimz/.initial=3,
  scale/.initial=1,
  densityx/.initial=1,
  densityy/.initial=1,
  densityz/.initial=1,
  rotation/.initial=0,
  anglex/.initial=0,
  angley/.initial=90,
  anglez/.initial=225,
  scalex/.initial=1,
  scaley/.initial=1,
  scalez/.initial=0.5,
%  drawxmarks/.is if=cuboiddrawxmarks,
%  drawymarks/.is if=cuboiddrawymarks,
  front/.style={draw=black,fill=white},
  top/.style={draw=black,fill=white},
  right/.style={draw=black,fill=white},
  drawfront/.is if=cuboiddrawfront,
  drawtop/.is if=cuboiddrawtop,
  drawright/.is if=cuboiddrawright,
  shade/.is if=cuboidshade,
  shadecolordark/.initial=black,
  shadecolorlight/.initial=white,
  shadeopacity/.initial=0.15,
  shadesamples/.initial=16,
  emphedge/.is if=cuboidemphedge,
  emphstyle/.style={thick},
  labels/.is if=cuboidlabels,
  frontpic/.is if=cuboidfrontpic,
  frontpicfp/.initial="",
  cuboidlabel/.initial="",
  ytextoff/.initial=0,
  ztextoff/.initial=0,
}

\newcommand{\tikzcuboidkey}[1]{\pgfkeysvalueof{/tikz/cuboid/#1}}

% Commands
\newcommand{\tikzcuboid}[1]{
    \tikzset{cuboid,#1} % Process Keys passed to command
  \pgfmathsetlengthmacro{\vectorxx}{\tikzcuboidkey{scalex}*cos(\tikzcuboidkey{anglex})*28.452756}
  \pgfmathsetlengthmacro{\vectorxy}{\tikzcuboidkey{scalex}*sin(\tikzcuboidkey{anglex})*28.452756}
  \pgfmathsetlengthmacro{\vectoryx}{\tikzcuboidkey{scaley}*cos(\tikzcuboidkey{angley})*28.452756}
  \pgfmathsetlengthmacro{\vectoryy}{\tikzcuboidkey{scaley}*sin(\tikzcuboidkey{angley})*28.452756}
  \pgfmathsetlengthmacro{\vectorzx}{\tikzcuboidkey{scalez}*cos(\tikzcuboidkey{anglez})*28.452756}
  \pgfmathsetlengthmacro{\vectorzy}{\tikzcuboidkey{scalez}*sin(\tikzcuboidkey{anglez})*28.452756}
  \newcommand{\frontpicfp}{\tikzcuboidkey{frontpicfp}}
  \begin{scope}[xshift=\tikzcuboidkey{shiftx}, yshift=\tikzcuboidkey{shifty}, scale=\tikzcuboidkey{scale}, rotate=\tikzcuboidkey{rotation}, x={(\vectorxx,\vectorxy)}, y={(\vectoryx,\vectoryy)}, z={(\vectorzx,\vectorzy)}]
    \pgfmathsetmacro{\steppingx}{1/\tikzcuboidkey{densityx}}
  \pgfmathsetmacro{\steppingy}{1/\tikzcuboidkey{densityy}}
  \pgfmathsetmacro{\steppingz}{1/\tikzcuboidkey{densityz}}
  \newcommand{\dimx}{\tikzcuboidkey{dimx}}
  \newcommand{\dimy}{\tikzcuboidkey{dimy}}
  \newcommand{\dimz}{\tikzcuboidkey{dimz}}
  \pgfmathsetmacro{\secondx}{2*\steppingx}
  \pgfmathsetmacro{\secondy}{2*\steppingy}
  \pgfmathsetmacro{\secondz}{2*\steppingz}
  \pgfmathsetmacro{\halfdimx}{0.5*\dimx}
  \pgfmathsetmacro{\halfdimy}{0.5*\dimy}
  % Draw front.
  \ifcuboiddrawfront
  \foreach \x in {\steppingx,\secondx,...,\dimx}
  { \foreach \y in {\steppingy,\secondy,...,\dimy}
    {   \pgfmathsetmacro{\lowx}{(\x-\steppingx)}
      \pgfmathsetmacro{\lowy}{(\y-\steppingy)}
      \filldraw[cuboid/front] (\lowx,\lowy,\dimz) -- (\lowx,\y,\dimz) -- (\x,\y,\dimz) -- (\x,\lowy,\dimz) -- cycle;
    }
  }
  \else
  \filldraw[cuboid/front] (0,0,\dimz) -- (0,\dimy,\dimz) -- (\dimx,\dimy,\dimz) -- (\dimx,0,\dimz) -- cycle;
  \fi
  \node [draw,opacity=0] (\tikzcuboidkey{cuboidlabel}) at (\halfdimx,\halfdimy,\dimz) {};
  % Draw top.
  \ifcuboiddrawtop
  \foreach \x in {\steppingx,\secondx,...,\dimx}
  { \foreach \z in {\steppingz,\secondz,...,\dimz}
    {   \pgfmathsetmacro{\lowx}{(\x-\steppingx)}
      \pgfmathsetmacro{\lowz}{(\z-\steppingz)}
      \filldraw[cuboid/top] (\lowx,\dimy,\lowz) -- (\lowx,\dimy,\z) -- (\x,\dimy,\z) -- (\x,\dimy,\lowz) -- cycle;
    }
  }
  \else
  \filldraw[cuboid/top] (0,\dimy,0) -- (0,\dimy,\dimz) -- (\dimx,\dimy,\dimz) -- (\dimx,\dimy,0);
  \fi
  % Draw right.
  \ifcuboiddrawright
  \foreach \y in {\steppingy,\secondy,...,\dimy}
  { \foreach \z in {\steppingz,\secondz,...,\dimz}
    {   \pgfmathsetmacro{\lowy}{(\y-\steppingy)}
      \pgfmathsetmacro{\lowz}{(\z-\steppingz)}
      \filldraw[cuboid/right] (\dimx,\lowy,\lowz) -- (\dimx,\lowy,\z) -- (\dimx,\y,\z) -- (\dimx,\y,\lowz) -- cycle;
    }
  }
  \else
  \filldraw[cuboid/right] (\dimx,0,0) -- (\dimx,0,\dimz) -- (\dimx,\dimy,\dimz) -- (\dimx,\dimy,0);
  \fi
  \ifcuboidemphedge
    \draw[cuboid/emphstyle] (0,\dimy,0) -- (\dimx,\dimy,0) -- (\dimx,\dimy,\dimz) -- (0,\dimy,\dimz) -- cycle;%
    \draw[cuboid/emphstyle] (0,\dimy,\dimz) -- (0,0,\dimz) -- (\dimx,0,\dimz) -- (\dimx,\dimy,\dimz);% Front
    \draw[cuboid/emphstyle] (\dimx,\dimy,0) -- (\dimx,0,0) -- (\dimx,0,\dimz);%
    \fi

    \ifcuboidshade
    \pgfmathsetmacro{\cstepx}{\dimx/\tikzcuboidkey{shadesamples}}
    \pgfmathsetmacro{\cstepy}{\dimy/\tikzcuboidkey{shadesamples}}
    \pgfmathsetmacro{\cstepz}{\dimz/\tikzcuboidkey{shadesamples}}
    \foreach \s in {1,...,\tikzcuboidkey{shadesamples}}
    {   \pgfmathsetmacro{\lows}{\s-1}
        \pgfmathsetmacro{\cpercent}{(\lows)/(\tikzcuboidkey{shadesamples}-1)*100}
        \fill[opacity=\tikzcuboidkey{shadeopacity},color=\tikzcuboidkey{shadecolorlight}!\cpercent!\tikzcuboidkey{shadecolordark}] (0,\s*\cstepy,\dimz) -- (\s*\cstepx,\s*\cstepy,\dimz) -- (\s*\cstepx,0,\dimz) -- (\lows*\cstepx,0,\dimz) -- (\lows*\cstepx,\lows*\cstepy,\dimz) -- (0,\lows*\cstepy,\dimz) -- cycle;
        \fill[opacity=\tikzcuboidkey{shadeopacity},color=\tikzcuboidkey{shadecolorlight}!\cpercent!\tikzcuboidkey{shadecolordark}] (0,\dimy,\s*\cstepz) -- (\s*\cstepx,\dimy,\s*\cstepz) -- (\s*\cstepx,\dimy,0) -- (\lows*\cstepx,\dimy,0) -- (\lows*\cstepx,\dimy,\lows*\cstepz) -- (0,\dimy,\lows*\cstepz) -- cycle;
        \fill[opacity=\tikzcuboidkey{shadeopacity},color=\tikzcuboidkey{shadecolorlight}!\cpercent!\tikzcuboidkey{shadecolordark}] (\dimx,0,\s*\cstepz) -- (\dimx,\s*\cstepy,\s*\cstepz) -- (\dimx,\s*\cstepy,0) -- (\dimx,\lows*\cstepy,0) -- (\dimx,\lows*\cstepy,\lows*\cstepz) -- (\dimx,0,\lows*\cstepz) -- cycle;
    }
    \fi
  % Labels.
  \ifcuboidlabels
    \pgfmathsetmacro{\botlabelx}{0.5*\dimx};
    %\draw[cuboid/emphstyle] (\botlabelx,0,\dimz) -- (\botlabelx,\dimy,\dimz) -- (0,0,\dimz); %   Debug.
    \draw (\botlabelx,0,\dimz) node [below] {\dimx};
    \pgfmathsetmacro{\leftlabely}{0.5*\dimy+\tikzcuboidkey{ytextoff}};
    \draw (0,\leftlabely,\dimz) node [left] {\dimy};
    \pgfmathsetmacro{\depthlabelz}{0.5*\dimz+\tikzcuboidkey{ztextoff}};
    \draw (\dimx,0,\depthlabelz) node [right] {\dimz};  
    % \node[draw] at (\botlabelx,0,\dimz) {some text spanning three lines with automatic line breaks};
    % Offset correction (nodes change parent node size, so the center is moved without this).
    \draw [opacity=0] (\botlabelx,\dimy,\dimz) node [above] {\dimz};
    \draw [opacity=0] (\dimx,\leftlabely,\dimz) node [right] {\dimy};
    \fi
   % Front picture.
   \ifcuboidfrontpic
     \pgfmathsetmacro{\frontw}{\dimx*\tikzcuboidkey{scalex}}
     \pgfmathsetmacro{\fronth}{\dimy*\tikzcuboidkey{scaley}}
     \pgfmathsetmacro{\ximpos}{0.5*\dimx};
     \node[canvas is xy plane at z=\dimz, transform shape, above, inner sep=0cm] at (\ximpos,0,0) {\includegraphics[width=\frontw cm,height=\fronth cm]{\frontpicfp}};
     %\draw (0,0,\dimz) node [canvas is xy plane at z=\dimz, transform shape]{\includegraphics[width=2cm,height=3cm]{\frontpicfp}}; \\
      \fi
  \end{scope}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Blob.
\newif\ifbloblabels
\newif\ifblobfrontpic
\tikzset{
  blob/.is family,
  blob,
  dimx/.initial=64,
  dimy/.initial=64,
  dimz/.initial=3,
  labels/.is if=bloblabels,
  frontpic/.is if=blobfrontpic,
  frontpicfp/.initial="",
  bloblabel/.initial="",
  ytextoff/.initial=0,
  ztextoff/.initial=0,
}
\newcommand{\tikzblobkey}[1]{\pgfkeysvalueof{/tikz/blob/#1}}
\newcommand{\blob}[1]{%
\tikzset{blob,#1}  % Process options.
  \pgfmathsetmacro{\scalex}{max(0.1/\tikzblobkey{dimx},log10(\tikzblobkey{dimx})/\tikzblobkey{dimx})*0.5}
  \pgfmathsetmacro{\scaley}{max(0.1/\tikzblobkey{dimy},log10(\tikzblobkey{dimy})/\tikzblobkey{dimy})*0.5}
  \pgfmathsetmacro{\scalez}{max(0.1/\tikzblobkey{dimz},.5*log10(\tikzblobkey{dimz})/\tikzblobkey{dimz})*0.5}
  \pgfmathsetmacro{\ytextoff}{\tikzblobkey{ytextoff}/\scaley}
  \pgfmathsetmacro{\ztextoff}{\tikzblobkey{ztextoff}/\scalez}
  \ifblobfrontpic
    \tikzcuboid{%
    dimx=\tikzblobkey{dimx},%
    dimy=\tikzblobkey{dimy},%
    dimz=\tikzblobkey{dimz},%
    scalex=\scalex,%
    scaley=\scaley,%
    scalez=\scalez,%
    front/.style={draw=none,fill=white},%
    top/.style={draw=none,fill=white},%
    right/.style={draw=none,fill=white},%
    emphedge=true,%
    labels=true,%
    frontpic=true,%
    frontpicfp=\tikzblobkey{frontpicfp},%
    cuboidlabel=\tikzblobkey{bloblabel},%
    ytextoff=\ytextoff,%
    ztextoff=\ztextoff,%
  }\\
     \else
    \tikzcuboid{%
    dimx=\tikzblobkey{dimx},%
    dimy=\tikzblobkey{dimy},%
    dimz=\tikzblobkey{dimz},%
    scalex=\scalex,%
    scaley=\scaley,%
    scalez=\scalez,%
    front/.style={draw=none,fill=white},%
    top/.style={draw=none,fill=white},%
    right/.style={draw=none,fill=white},%
    emphedge=true,%
    labels=true,%
    cuboidlabel=\tikzblobkey{bloblabel},%
    ytextoff=\ytextoff,%
    ztextoff=\ztextoff,%
  }\\
  \fi
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> sections/future_work.tex <==
Instead of color, these cues could consist of edges / wrinkles or any other localized conditioning.
An alternative way to enforce conditioning could be, to add a loss on certain parts of the latent encoding vector to enforce correlation with external attributes~\cl{ref}. %NL%
This could be used to, e.g., enforce the presence of a certain type of clothing.
